On a Uniform Causality Model for Industrial Automation

The increasing complexity of Cyber-Physical Systems (CPS) makes industrial automation challenging. Large amounts of data recorded by sensors need to be processed to adequately perform tasks such as diagnosis in case of fault. A promising approach to deal with this complexity is the concept of causality. However, most research on causality has focused on inferring causal relations between parts of an unknown system. Engineering uses causality in a fundamentally different way: complex systems are constructed by combining components with known, controllable behavior. As CPS are constructed by the second approach, most data-based causality models are not suited for industrial automation. To bridge this gap, a Uniform Causality Model for various application areas of industrial automation is proposed, which will allow better communication and better data usage across disciplines. The resulting model describes the behavior of CPS mathematically and, as the model is evaluated on the unique requirements of the application areas, it is shown that the Uniform Causality Model can work as a basis for the application of new approaches in industrial automation that focus on machine learning.

==> Kommentare.tex <==
Intro

-> better introduce CPS

requirements

-> requirements not well motivated
-> not formalized properly

Literature

-> misunderstandings! more thorough literature review necessary

-> "I am not sure what section 2 wants to introduce and how it
serves the paper. Moreover, many statements and summaries
can be misleading and ambiguous”

-> causal inference vs causal discovery
-> causal inference assumes a causal graph is known
-> it is causal structure learning/causal discovery that assumes there is no knowledge

-> we are more closely related to causal RepL (data-driven) and try to pimp it with compositional knowledge. However, causal inference is the much bigger research community

-> we must locate our proposal more precisely

-> literature focuses on data driven and probailistic approaches, ignores “huge amount of work on this topic done in [symbolic?] AI”
action and change in the KR&R (knowledge representation & reasoning) community, especially qualitative reasoning

-> qualitative process theory by Forbus

Definitions/Model

->too close to standard automation theory

-> stochastic processes necessary?

-> how to define a “forced distribution shift”?

-> formal definition UCM missing

-> too general? Where is the specific context to CPS? perhaps sensors. However reliance on sensors, sensor data system. Sensor data can be added/removed or faulty, but this does not change underlying causality
rebuttal:
causality in itself is not measurable, sensors enable learning a “best guess” about the system’s causal structure of course, this observed model differs from the “real” causal model, however, the real causal model has an effect on the physical properties of the model, which is measurable via sensors. plus, humans learn similarly. make clearer that a causal model based on sensor data can be flawed but useful?

-> where is the CPS input/controls?
can be measured via sensors, actuators (with discrete distribution)
this has to be made clearer

-> Definition 1 (effect) “problematic” (?), compare to [Lozano-Durán, A., & Arranz, G.
(2022)]

-> what if components that are not observable are faulty? → consistency-based
diagnosis can work with that
Kommentar Lukas: Es wird in einem Satz  gesagt "computing the root cause of a fault based on potentially incomplete observations". 
Hier sonst im state of the art nochmal eine Quelle nennen?
(An improved diagnostic method for probabilistic consistency-based diagnosis, Marcos L. P. Bueno1, Arjen Hommersom, and Peter J. F. Lucas)



minor

-> Def. 3: here, refers to the set of all sensor *values*; right after Def. 2, the
same letter denotes the set of all sensors

-> deterministic? → well-defined

Applications

-> illustrative examples?!

-> give algorithm

-> case study on real use-case!

-> consistency-based diagnosis
Kommentar Lukas: Einfügen von consistency based Diagnosis (SOTA Line 100) mit zB den Quellen: 
- Johan de Kleer and Brian C. Williams. Diagnosing multiple faults.
- An improved diagnostic method for probabilistic consistency-based diagnosis, Marcos L. P. Bueno, Arjen Hommersom, and Peter J. F. Lucas
 Text: Consistency-based diagnosis belongs to the weak fault approach. Here, the consistency of the system is checked by comparing the learned model of normal behavior against the actual behavior. Inconsistency between observable components can be detected and a diagnosis of the system can be performed on this basis. For accurate identification of the fault, a sufficient number of observable components is important. However, if there are only partial observable components [Bueno] proposed the diagnostic coefficient that uses the likelihood of the observations as the basis of discrepancy indicator to solve this partial observability case.


-> fault signatures? mode signatures?

-> local faults based on components, which have to be put together via compositionality however, this has to be done manually

-> learning the CPS structure based on plans actually feasible? We justcite some research, but it is not well integrated with our model

-> what is the benefit for ML?

Evaluation

-> evaluation missing, has to be based on application
“the authors do not succeed in convincingly demonstrating the
actual and practical usefulness of the model”

-> is supposed to be based on requirements, but they are too general and not well motivated

Other
-> Casuality may be different depending on the entity. […] How does the proposed theory deal with mass/energy equations???

additional comments CRL

-> P1: “A definition of causality in CPS would be beneficial for using causality in the context of machine learning.“
it requires a justification for why so.

-> P1: “However, causality has only recently seen increased attention [Schölkopf et al., 2021]”

-> P1: “Causality is often represented in graphs, namely Directed Acyclic Graphs (DAGs) [Pearl, 1995]. DAGs do not allow cycles, which means they do not allow relations such as A influencing B and B influencing A.”
Note that there are works on the cyclic causal graphs. It would avoid misleading by including these works.

-> P2: “Requirement 8: Components may be OK or not-OK (KO).”

-> P2: “Causality is often analyzed using the approach of causal inference.”

-> P2: “As causal relations cannot be directly read off from the data, they have to be inferred by settings such as randomized control trials, where the randomization counteracts confounding factors [Eberhardt, 2017].”

-> P2: “Furthermore, modeling approaches such as state machines encode causal knowledge and can be executed to compare the behavior of the simulated system with real-world data.”; ”Causal dependencies can be inferred from plant documentation to extract engineering information about the plant and from process data.”
I am not sure that I am familiar with this and didn’t understand how it getsthe causal dependencies.

-> P2: “In industrial automation, an application closely connected to causality is the planning of a production process, which deals with the order of functionalities within the process to produce a certain product.” “Since causalities are the basis for the transformations,”
What does the causality mean here ? --> lass ich mir noch was einfallen --> check
Problem ist glaube ich, dass nicht klar wird, dass wir von unterschiedlichen leveln reden und vllt/anscheinend nicht hinreichend klar wird, dass für uns kausalität eben nicht nur diagnose ist. sondern dass wir darunter generell einen kausalen Zusammenhang verstehen. in diesem fall halt, die Transformaion eines Produktes, die durch eine Aktion verursacht wird. 

-> P2: “Within recent years the AI planning community developed approaches to use so called action model learning for AI planning.”
Some citations here can be helpful. -> Check 

-> P3: “Despite the existing theoretical approaches of AI planning, there are no concrete and successful implementations in industrial automation so far since real world planning problems are very complex and the prerequisites, such as a modular CPPS, have not yet been created.” -> Check

-> P3 “Such systems are difficult to learn, since it is not only required to capture the temporal dependency of each time series, but causal relations between different pairs of time series [Zhang et al., 2019].”
I am not sure “since” is proper for the logic of the sentence.

additional comments DX

ADDITIONAL COMMENTS:
-> Sec. 1: the first two sentences seem a bit redundant, please improve

-> at last so-far --> at least so far

-> Sec. 1, last paragraph: Arabic numbers should be used instead of roman ones to refer to the paper's sections

-> Def. 3: here, \mathcal{Y} refers to the set of all sensor *values*; right after Def. 2,
the same letter denotes the set of all sensors

-> Sec. 3.1: what does "deterministic" formally mean for a function? Do you mean well-defined, i.e., that it always maps one and the same value to one and the same image? Or do you mean injective, i.e., that different inputs always yield different
images? Please use a commonly known terminology or formally define/explain what you mean

-> I did not understand inter alia the following passages:
-- last sentence of page 1, right column, 3rd paragraph
-- "Where to separate a causal chain..."
-- "Multiple components form a web of causal chains, which might be considered a
module when the resulting subsystem forms a functional unit."
-- "(sub-)atomic level" -- what does this mean in this particular context?
-- last paragraph of Sec. 3.2

==> conclusion.tex <==
\section{Conclusion} \label{conclusion}

% Causality has been a focus of research in many areas for many decades. 
Modern approaches to causality mostly concern themselves with unraveling causal relations in unknown systems by analyzing large amounts of data. 
However, these approaches are not ideally suited for engineering applications, because they do not leverage knowledge about the hierarchical structure of CPS and fundamental behavior such as control circuits cannot be modeled.
% It is therefore useful and necessary to develop a concept of causality for the engineering field. 
%
Here, we present a first step towards the development of a formalism for causality in automation, specifically for analyzing, planning and diagnosing CPS and CPPS. We term this formalism the Uniform Causality Model. 
%
% The UCM mathematically defines causal relations between components in a CPS by defining the concepts of cause, effect, causal relation and subsystem. 
% Furthermore, the concept of causal construction is formalized. 
% To enable usage in the field of diagnosis, the concepts of state, faulty sensor and faulty components are also defined. 
We believe that the UCM is a valuable first step into developing a uniform approach to causality in all disciplines of automation. 
